Learning Locally Editable Virtual Humans

In this paper, we propose a novel hybrid representation and end-to-end trainable network architecture to model fully editable and customizable neural avatars. At the core of our work lies a representation that combines the modeling power of neural fields with the ease of use and inherent 3D consistency of skinned meshes. To this end, we construct a trainable feature codebook to store local geometry and texture features on the vertices of a deformable body model, thus exploiting its consistent topology under articulation. This representation is then employed in a generative auto-decoder architecture that admits fitting to unseen scans and sampling of realistic avatars with varied appearances and geometries. Furthermore, our representation allows local editing by swapping local features between 3D assets. To verify our method for avatar creation and editing, we contribute a new high-quality dataset, dubbed CustomHumans, for training and evaluation. Our experiments quantitatively and qualitatively show that our method generates diverse detailed avatars and achieves better model fitting performance compared to state-of-the-art methods. Our code and dataset are available at https://custom-humans.github.io/.

==> main/FIG_cross_subjects.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{images/cross_subjects.pdf}
\caption{\textbf{Exemplar of cross subjects local feature control}.}
\label{fig:random}
\end{figure}

==> main/FIG_customization.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{images/main_results2.pdf}
\caption{\textbf{Avatar customization pipeline}. Two exemplars of avatar creation using our proposed framework. (a) Starting from a random body geometry and texture (\emph{Top}) or training sample saved in our feature dictionary (\emph{Bottom}), we keep human identities (i.e., face textures, geometries) unchanged while gradually (b) editing new clothing geometry and (c) textures onto our avatar by fitting to unseen 3D scans and 2D images. (d) Note that our method can handle challenging loose clothing such as jackets and coats and keep their colors and geometries consistent under various poses. }
\label{fig:main}
\end{figure*}

==> main/FIG_repose.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.9\linewidth]{images/reposing.pdf}
\caption{\textbf{Qualitative analysis of reposing on CustomHumans}. We visualize the results of avatar reposing using different percentages of training data (i.e., 10 meshes vs 100 meshes). Artifacts caused by self-contact (e.g., fist and elbow) can be reduced when more training subjects are introduced.}
\label{fig:data_repose}
\end{figure}

==> main/FIG_training.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{images/sampling.pdf}
\caption{\textbf{Two codebook sampling protocols for training.} \emph{Top}: Given a random subject index, we query the corresponding codebook stored in the dictionary. This \textbf{queried codebook} is used for 3D supervision, and its gradients \emph{do not} back-propagate to the whole dictionary. \emph{Bottom}: We apply PCA to the high-dimensional dictionary, and draw a random sample in the $D$-dimensional PCA space. As the \textbf{sampled codebook} is a combination of the PCA eigenvectors, the 2D adversarial loss will be used for updating the whole dictionary. Note that both strategies are applied during training to jointly optimize the dictionaries and decoders. }
\label{fig:training}
\end{figure}

==> main/TAB_Feature_query.tex <==
\begin{table}[t]
    \centering
\begin{tabular}{l|c|c}
\hline
                                  & Scan-to-Pred & Pred-to-Scan     \\
\hline
 NN                            & 0.456 & 0.668 (-45.6\%)           \\
 KNN-weighted sum                & 0.474 & 1.980 (\textbf{-317.7\%})  \\
 Ours                               & 0.474 & 1.980 (\textbf{-317.7\%})  \\
\hline
\end{tabular}
\caption{\textbf{Quantitative comparison of model fitting}. We report ...}
\label{tab:fitting}
\end{table}

==> main/TAB_dataset.tex <==
\begin{table}[t]
    \centering
\begin{tabular}{lcccc}
\toprule
  Dataset         & \begin{tabular}[c]{@{}c@{}} \# Scans \\ / Subjects \end{tabular}   & Watertight  & Noise  & \begin{tabular}[c]{@{}c@{}} Publicly \\ Available \end{tabular}       \\
\midrule
 \begin{tabular}[l]{@{}l@{}} Commercial \\ Data \end{tabular} &  N/A      & Yes    &  No           & No        \\
 SIZER                &   2000+ / 22             & No     &  Yes        &      Yes  \\
 THuman2.0            &   500+ / 150+            & Yes    &  Yes        &      Yes  \\
 Ours                 &  1000+ /100              & Yes    &  No         &       Yes  \\
\bottomrule
\end{tabular}
\caption{\textbf{Summary of existing 3D human scans datasets}. }
\label{tab:fid}
\end{table}
